Machine Translation Models Stand Strong in the Face of Adversarial Attacks

Adversarial attacks expose vulnerabilities of deep learning models by introducing minor perturbations to the input, which lead to substantial alterations in the output. Our research focuses on the impact of such adversarial attacks on sequence-to-sequence (seq2seq) models, specifically machine translation models. We introduce algorithms that incorporate basic text perturbation heuristics and more advanced strategies, such as the gradient-based attack, which utilizes a differentiable approximation of the inherently non-differentiable translation metric. Through our investigation, we provide evidence that machine translation models display robustness displayed robustness against best performed known adversarial attacks, as the degree of perturbation in the output is directly proportional to the perturbation in the input. However, among underdogs, our attacks outperform alternatives, providing the best relative performance. Another strong candidate is an attack based on mixing of individual characters.

==> app.tex <==
\section{Machine Translation Attack Examples}
\label{app_b}

\begin{table*}[h!]
\centering
% \begin{tabular}{p{1.5cm}p{3cm}p{10.5cm}}
\begin{tabular}{p{1.5cm}p{3cm}p{7.5cm}}
Attack type & Sentence type & Sentence \\ \cline{1-3} 
Gradient &  Orig. sentence & Cars get many more miles to the gallon. \\   \cline{2-3} 
&         Attacked sentence &  Cars get many more miles to the \textcolor{red}{ormoneon}. \\   \cline{2-3} 
&         Orig. translation & Автомобили проезжают больше миль на один галлон. \\   \cline{2-3} 
&         Translation & Машины проехали еще много миль до галлона. \\   \cline{2-3} 
&         Attacked translation & Машины проехали гораздо больше миль до гормона. \\ 

\hline

BLEUER &    Orig. sentence & Cars get many more miles to the gallon. \\   \cline{2-3} 
&         Attacked sentence & Cars get many more miles to the \textcolor{red}{gall }on. \\   \cline{2-3} 
&         Orig. translation & Автомобили проезжают больше миль на один галлон. \\   \cline{2-3} 
&         Translation & Автомобили получают гораздо больше миль до галлона. \\   \cline{2-3} 
&         Attacked translation & Автомобили получают гораздо больше миль до галлона. \\   \cline{1-3}

\hline

Synthetic &         Orig. sentence & Cars get many more miles to the gallon. \\   \cline{2-3} 
&         Attacked sentence & \textcolor{red}{arCs egt myna emro ielsm to het gllnoa.} \\   \cline{2-3} 
&         Orig. translation & Автомобили проезжают больше миль на один галлон. \\   \cline{2-3} 
&         Translation & Машины проехали еще много миль до галлона. \\   \cline{2-3} 
&         Attacked translation & arCs eggt myna empro ielsm to het glnoa. \\   \cline{1-3}

\hline
\end{tabular}
\caption{Attack samples for the Machine Translation task for different types of attacks.}
\label{table:attack_samples_mt_grad}
\end{table*}

\newpage




==> appb.tex <==
\chapter{Machine Translation Attack Examples}
\label{app_b}

\begin{table*}[h!]
\centering
\begin{tabular}{p{1.5cm}p{3cm}p{10.5cm}}
Attack type & Sentence type & Sentence \\ \cline{1-3} 
Gradient &         Orig. sentence & The push comes as the country's Highway Trust Fund, financed with taxes Americans pay at the gas pump, is broke. \\   \cline{2-3} 
&         Attacked sentence &  The \textcolor{red}{pushed come as} the country's \textcolor{red}{ROAD} Trust Fund, financed with taxes Americans pay at the gas \textcolor{red}{pumps}, is \textcolor{red}{break}. \\   \cline{2-3} 
&         Orig. translation & Необходимость этого усугубляется отсутствием средств у Правительственного Фонда строительства шоссейных дорог, финансируемого за счёт налогов, которые американцы платят на автозаправках. \\   \cline{2-3} 
&         Translation & Толчок приходит к тому, что Целевой фонд для автомобильных дорог, финансируемый за счет налогов, которые американцы платят за газовый насос, разоряется. \\   \cline{2-3} 
&         Attacked translation & Толчка приходит, как Дорожный целевой фонд страны, финансируемый за счет налогов, которые американцы платят за газовые насосы, ломается. \\   \cline{1-3} 

&         Orig. sentence & Americans don't buy as much gas as they used to. \\   \cline{2-3} 
&         Attacked sentence &  Americans don't \textcolor{red}{bought as} much \textcolor{red}{gases} as they used to. \\   \cline{2-3} 
&         Orig. translation & Американцы уже не покупают так много бензина, как раньше. \\   \cline{2-3} 
&         Translation & Американцы покупают не столько бензина, сколько раньше. \\   \cline{2-3} 
&         Attacked translation & Американцы купили не столько газов, сколько раньше. \\   \cline{1-3} 

&         Orig. sentence & Cars get many more miles to the gallon. \\   \cline{2-3} 
&         Attacked sentence &  Cars get many more miles to the \textcolor{red}{ormoneon}. \\   \cline{2-3} 
&         Orig. translation & Автомобили проезжают больше миль на один галлон. \\   \cline{2-3} 
&         Translation & Машины проехали еще много миль до галлона. \\   \cline{2-3} 
&         Attacked translation & Машины проехали гораздо больше миль до гормона. \\ 

\bottomrule 
\end{tabular}
\caption{Attack samples for Machine Translation task for gradient attack.}
\label{table:attack_samples_mt_grad}
\end{table*}

\newpage


\begin{table*}[h!]
\centering
\begin{tabular}{p{1.5cm}p{3cm}p{10.5cm}}
Attack type & Sentence type & Sentence \\ \cline{1-3} 
BLEUER &         Orig. sentence & The push comes as the country's Highway Trust Fund, financed with taxes Americans pay at the gas pump, is broke. \\   \cline{2-3} 
&         Attacked sentence & The push\textcolor{red}{eshed} comes as the country's Highway Trust Fund, financed with taxes Americans pay at the gas pump, is broke. \\   \cline{2-3} 
&         Orig. translation & Необходимость этого усугубляется отсутствием средств у Правительственного Фонда строительства шоссейных дорог, финансируемого за счёт налогов, которые американцы платят на автозаправках. \\   \cline{2-3} 
&         Translation & Надвиг наступил, так как в стране Highway Trust Fund, финансируемый налогами, которые американцы платят на насосе газа, развалился. \\   \cline{2-3} 
&         Attacked translation & Надвиг наступил, так как фонд Highway Trust Fund, финансируемый налогоплательщиками, которые платят на насосе газа, развалился. \\   \cline{1-3} 

&         Orig. sentence & Americans don't buy as much gas as they used to. \\   \cline{2-3} 
&         Attacked sentence & Americans don't buy as much \textcolor{red}{fuel} as they used to. \\   \cline{2-3} 
&         Orig. translation & Американцы уже не покупают так много бензина, как раньше. \\   \cline{2-3} 
&         Translation & Американцы не покупают столько газа, сколько раньше. \\   \cline{2-3} 
&         Attacked translation & Американцы не покупают столько газа, сколько раньше. \\   \cline{1-3} 

&         Orig. sentence & Cars get many more miles to the gallon. \\   \cline{2-3} 
&         Attacked sentence & Cars get many more miles to the \textcolor{red}{gall }on. \\   \cline{2-3} 
&         Orig. translation & Автомобили проезжают больше миль на один галлон. \\   \cline{2-3} 
&         Translation & Автомобили получают гораздо больше миль до галлона. \\   \cline{2-3} 
&         Attacked translation & Автомобили получают гораздо больше миль до галлона. \\   \cline{1-3} 

\bottomrule 
\end{tabular}
\caption{Attack samples for Machine Translation task for "BLEUER" attack.}
\label{table:attack_samples_mt_bleuer}
\end{table*}

\newpage

\begin{table*}[h!]
\centering
\begin{tabular}{p{1.5cm}p{3cm}p{10.5cm}}
Attack type & Sentence type & Sentence \\ \cline{1-3} 
Synthetic &         Orig. sentence & The push comes as the country's Highway Trust Fund, financed with taxes Americans pay at the gas pump, is broke. \\   \cline{2-3} 
&         Attacked sentence & \textcolor{red}{heT push comes sa eth uocntry's giHhway trusT Fund, fcnanied iwth tesax Ameracisn yap ta het ags pump, si broek.} \\   \cline{2-3} 
&         Orig. translation & Необходимость этого усугубляется отсутствием средств у Правительственного Фонда строительства шоссейных дорог, финансируемого за счёт налогов, которые американцы платят на автозаправках. \\   \cline{2-3} 
&         Translation & Толчок приходит к тому, что Целевой фонд для автомобильных дорог, финансируемый за счет налогов, которые американцы платят за газовый насос, разоряется. \\   \cline{2-3} 
&         Attacked translation & Приближается фонд "Гихуэй Трус", Феннайд Текса Амерасин Яп Та Гет Агс насос, Си Брук. \\   \cline{1-3} 

&         Orig. sentence & Americans don't buy as much gas as they used to. \\   \cline{2-3} 
&         Attacked sentence & \textcolor{red}{Arnmicsea 'ontd ybu sa hmcu sag as teyh esud ot.} \\   \cline{2-3} 
&         Orig. translation & Американцы уже не покупают так много бензина, как раньше. \\   \cline{2-3} 
&         Translation & Американцы покупают не столько бензина, сколько раньше. \\   \cline{2-3} 
&         Attacked translation & Арммикси интуитивно ybu sa hmcu sag как teyh esud ot. \\   \cline{1-3} 

&         Orig. sentence & Cars get many more miles to the gallon. \\   \cline{2-3} 
&         Attacked sentence & \textcolor{red}{arCs egt myna emro ielsm to het gllnoa.} \\   \cline{2-3} 
&         Orig. translation & Автомобили проезжают больше миль на один галлон. \\   \cline{2-3} 
&         Translation & Машины проехали еще много миль до галлона. \\   \cline{2-3} 
&         Attacked translation & arCs eggt myna empro ielsm to het glnoa. \\   \cline{1-3} 

\bottomrule 
\end{tabular}
\caption{Attack samples for Machine Translation task for Synthetic attack.}
\label{table:attack_samples_mt_bleuer}
\end{table*}
